Secure Distributed Training at Scale

Many areas of deep learning benefit from using increasingly larger neural networks trained on public data, as is the case for pre-trained models for NLP and computer vision. Training such models requires a lot of computational resources (e.g., HPC clusters) that are not available to small research groups and independent researchers. One way to address it is for several smaller groups to pool their computational resources together and train a model that benefits all participants. Unfortunately, in this case, any participant can jeopardize the entire training run by sending incorrect updates, deliberately or by mistake. Training in presence of such peers requires specialized distributed training algorithms with Byzantine tolerance. These algorithms often sacrifice efficiency by introducing redundant communication or passing all updates through a trusted server, making it infeasible to apply them to large-scale deep learning, where models can have billions of parameters. In this work, we propose a novel protocol for secure (Byzantine-tolerant) decentralized training that emphasizes communication efficiency.

==> backup_related_byzantine.tex <==

\textbf{Extremely useful survey-paper: \cite{lyu2020privacy}.} It contains a huge number of references. Almost all we need is cited there. Good feature: it contains a separate section on Sybil attacks.

\begin{itemize}
    \item Parameter-server (PS) acrhitecture (all papers in this part rely significantly on the existense of PS)
    \begin{itemize}
        \item \algname{Momentum-SGD} with \algname{CenteredClip} aggregation \cite{karimireddy2020learning}. This is a central paper for us. Explains why popular ``robust'' aggregation rules and permutation invariant methods are not good enough against byzantines. Good convergence guarantees in the non-convex case (for finding first-order stationary points). Communication cost: 1 vector from each node per iteration.
        \item \algname{SafeguardSGD} \cite{allen2020byzantine}. Interesting approach (perturbed \algname{SGD} with statistical tests based on the statistical concentration), but it was analyzed under too restrictive assumptions (almost surely bounded noise). Some convergence guarantees in the non-convex case for finding second-order stationary points. Good description of the popular attacks. Communication cost: 1 vector from each node per iteration. This paper is a follow-up of \cite{alistarh2018byzantine} where the authors considered very similar method -- \algname{ByzantineSGD}. However, they also use too restrictive assumption.
        \item Byzantine-tolerant \algname{SAGA} (variance-reduced version of \algname{SGD}) \cite{wu2020federated}. The paper is based on the following observation: since the variance becomes smaller during the optimization process it becomes increasingly simpler to identify byzantines and, therefore, with proper aggregation the method can converge with any predefined accuracy. It turns out that for \algname{SAGA} it is enough to use geometrical median as an aggregation rule. Communication cost: 1 vector from each node per iteration. Recently, this paper was generalized: communication compression was added to the method \cite{zhu2021broadcast}. Communication cost: 1 compressed vector from each node per iteration. The main drawback is that variance-reduced methods are known to behave worse than simple \algname{SGD} on training the deep learning models \cite{defazio2018ineffectiveness}. Moreover, one needs to solve an auxiliary problem at each iteration to find geometrical median.
        \item \algname{SGD} with \algname{Krum} aggregator \cite{blanchard2017machine}. Classical paper, beaten by many other approaches.
        \item \algname{SGD} with coordinate-wise median and trimmed coordinate-wise median \cite{yin2018byzantine}. Classical paper, beaten by many other approaches.
        \item \algname{Multi-Krum} \cite{damaskinos2019aggregathor}. No convergence guarantees.
        \item \algname{Bulyan} \cite{mhamdi2018hidden}. Special aggregation rule based on the iterative application of some robust aggregation rule. Weak theory, following from \cite{blanchard2017machine}.
        \item Robust Federated Averaging (\algname{RFA}) \cite{pillutla2019robust}. In fact, it is just \algname{Local-SGD} with geometrical median averaging. There are some theoretical guarantees, but the contradict to the counter-examples from \cite{karimireddy2020learning}.
        \item \algname{Draco} \cite{chen2018draco}. This approach is based on the redundancy of the computations. Roughly speaking, one can eliminate byzantines by using redundant computations.
        \item \algname{Detox} \cite{rajput2019detox}. This approach can be applied on top of any robust aggregator. The idea is to use redundant computations in groups (one group of workers compute the stochastic gradient using the same batch), then PS uses majority vote, after that, the aggregation is performed in two steps.
        \item Some papers about the ineffectiveness of the classical byzantine tolerant aggregators as coordinate-wise median and Krum: \cite{baruch2019little,xie2020fall}. Some concrete examples of attacks that break Krum, median, trimmed median, Bulyan.
        \item Heuristic for ranking the workers in federated learning algorithms \cite{rodriguez2020dynamic}. No theory is provided. Moreover, it seems that their approach is not robust against simple attacks.
        \item Reputation scores + \algname{SGD} \cite{regatti2020bygars}. Interesting idea of dynamical updates of scores for workers. The authors proved almost sure convergence of their scheme (non-asymptotic rates are not given). The main issue with the analysis: it works only for multiplicative noise attacks, i.e., they assumed that byzantines always send $Const \times g^k$, where $g^k$ is the stochastic gradient. This assumption is too restrictive, e.g., it does not hold for label flipping attacks. Anyway, the idea is interesting.
        \item Reputations based on cosine measure between reputation-weighted average of gradients (weights = reputation scores) and workers' gradients + removing workers with too small reputation \cite{xu2020towards}. It seems, that one byznatine worker can break the work of their algorithm since the worker can send large vector that will make the cosine measure between his vector and the averaged vector big whereas for fair workers it will be negligible. That is, after 1 round all fair workers will be removed.
    \end{itemize}
    \item Decentralized architecture
    \begin{itemize}
        \item Byzantine-robust decentralized \algname{SGD} \cite{peng2021byzantine}. The approach is based on the interesting idea know long time ago in the signal processing community \cite{ben2013robust} (funny and strange fact: 0 citations in Google Scholar). That is, one can replace the original problem by TV-regularized problem with large enough regularization parameter $\lambda$ and solve it via \algname{Decentralized SGD}. One can easily show that for large enough regularization parameter the TV-regularized problem and the original problem are equivalent. However, there are several issues with this approach. First of all, in \cite{peng2021byzantine}, the authors showed the convergence only to some neighborhood of the solution. The size of the neighborhood cannot be reduce in general unless all functions on nodes are the same, which is meaningful, and, more importantly, unless $\lambda = 0$. However, when $\lambda = 0$ their algorithm reduces to running \algname{SGD} on good nodes without any communications. So, this is impractical for distributed training of large DL models. Nevertheless, I think, it would be useful to compare our method with their in numerical experiments (in theory, our algorithm is obviously better). The same idea was used in \cite{li2019rsa} where authors also use the approach with regularization but for parameter-server architecture.
        \item \algname{ByRDiE} \cite{yang2019byrdie} and \algname{BRIDGE} \cite{yang2019bridge}. Both papers are a little bit strange: they assume that workers compute the full gradients + they use trimmed coordinate-wise median that is provably bad against byzantine attacks. As the result they obtained useless algorithms: in heterogeneous case their defenses are suspicious since one cannot do anything against byzantines without heuristics as reputation scores and additional assumptions. Moreover, in homogeneous case, the algorithms are strange since all good workers already compute the full gradients of the loss. Therefore, in this case, they can work without communications.
    \end{itemize}
    \item Blockchain ?
    \item Communication overheads!
\end{itemize}
